Flash Inference: Near Linear Time Inference for Long Convolution Sequence Models and Beyond

While transformers have been at the core of most recent advancements in sequence generative models, their computational cost remains quadratic in sequence length. Several subquadratic architectures have been proposed to address this computational issue. Some of them, including long convolution sequence models (LCSMs), such as Hyena, address this issue at training time but remain quadratic during inference. We propose a method for speeding up LCSMs' exact inference to quasilinear $O(L\log^2L)$ time, identify the key properties that make this possible, and propose a general framework that exploits these. Our approach, inspired by previous work on relaxed polynomial interpolation, is based on a tiling which helps decrease memory movement and share computation. It has the added benefit of allowing for almost complete parallelization across layers of the position-mixing part of the architecture. Empirically, we provide a proof of concept implementation for Hyena, which gets up to $7.8\times$ end-to-end improvement over standard inference by improving $110\times$ within the position-mixing part.

==> 4-flash-inference/algo-section.tex <==
\subsection{The General Algorithm}
\label{sec:general-algorithm}

We derive inspiration from the the work of \citet{van1997initalFastCDQ} regarding relaxed polynomial interpolation - they propose a fix to dealing with \emph{dynamic} structure of \ref{onlineConv} to achieve an overall $O(L\log^2 L)$ times. While their work is specific to convolutions (and thus can only translate to LCSMs), their approach can be generalized to act as a static-to-dynamic translator. This comes at the price of blowing up FLOPs by just $\log L$ over the static procedure.
% \candelete{(that performs the desired computation if the input sequence is given all at once - as is the case with using FFT during training in LCSMs).}

In describing the method, we will constrain ourselves to the LCSM setting, but all of the reasoning can be applied more broadly. The high-level idea is to tile the contributions into chunks that can be dealt with by calls to $\gA$. However, as mentioned in Section \ref{the-inference-problem}, we need to be careful about the inputs being fully available at the time of calling $\gA$ and this is the main problem to solve.
% Schematically, the contribution tiling is depicted in Figure~\ref{fig:lazy-eager-fast-tiling} and the algorithm is shown in Algorithm~\ref{alg:flash-inference-lcsm}.

The crux of the algorithm is exploiting~\ref{assumption:query-independent}: particularly, one can start accounting for $\cont(y, i, j)$ as soon as $y_i$ becomes available - this is in contrast to transformers where $\cont(y, i, j)$ depends on $q_j$ which depends on $y_j$. Hence, one can do work ahead of time, at the very extreme accounting for $\cont(y, i, j)$ for all $j \geq i$ as soon as $y_i$ is computed. This eager approach, however, still scales quadratically in $L$ - the issue is that we are essentially incurring a cost of $\gT(1, L - i + 1)$. The standard (lazy) implementation, which at time $j$ iterates through all $i \leq j$ and accounts for their contribution essentially incurs a $\gT(j, 1)$ cost. As noted in Lemma~\ref{lemma:lcsm-block-fft}, by balancing the two inputs of $\gT$, one can use FFT to lower $\gT(L_1, L_2)$ significantly below $L_1\cdot L_2$ and this yields biggest improvements when $L_1$ and $L_2$ are balanced. This motivates the fractal tiling from Figure~\ref{fig:lazy-eager-fast-tiling}. This tiling is different from the one proposed by \citet{van1997initalFastCDQ} and saves a factor $2$ by exploiting the fact that $k$ is data-independent. However, as explored in Appendix~\ref{sec:data-dependent-filters-appendix}, one can use \citet{van1997initalFastCDQ}'s approach to work with data-dependent filters.

The algorithm is illustrated in Algorithm~\ref{alg:flash-inference-lcsm}. The outer loop (\ref{line:outer-loop}) iterates through positions $i$: at each iteration, one computes all the activations at position $i$, does some (limited) eager work and samples next token. To do so, the inner loop (\ref{line:inner-loop} iterates through the several mixer-layers. It first accounts for the red cells in the diagram, that is, the direct dependency on previous layer's activations at position $i$ (line~\ref{line:red-tile}). After computing the activation at position $i$, it also accounts for the contribution of the gray tile that has just been unlocked (line~\ref{line:gray-tile}) at the current layer - this is only useful to save compute in the long term, while not being immediately necessary to sample the next token. The accounting works for considering (in-place) the influence of last $U$ positions to next $U$ ones. For example, during iteration $i=6$, following the Figure~\ref{fig:lazy-eager-fast-tiling}, the gray cell has $5\leq i \leq 6$ and $7 \leq j \leq 8$, corresponding to $U = 2$ defined as largest power of $2$ that divides $i=6$. Importantly, one can only account for a tile (red or gray) once all its $i$'s are known at the previous layer.

==> algos/flash-lcsm-in-place.tex <==
\begin{algorithm}[ht]
\caption{Flash Inference for LCSMs in-place}
\label{alg:flash-inference-lcsm-in-place}
\begin{algorithmic}[1]
    \REQUIRE filter $\rho \in \mathbb{R}^{M \times L \times D}$, $\block^{[1, M]}$, first token $a_{1, 0}$ and $\sampler$
    \STATE \textbf{Output:} All activations $a_0, \ldots, a_M \in \mathbb{R}^{L \times D}$ obtained by autoregressively sampling
    \STATE Initialize $a$ with zeros outside $a_{1, 0}$
    \FOR{$i \leftarrow 1$ \textbf{to} $L-1$} \label{line:outer-loop}
        \STATE $U \leftarrow$ maximum power of $2$ that divides $i$ \text{  \# the side of the $i$\textsuperscript{th} gray tile} \label{line:define-tile-side}
        \FOR{$\ell \leftarrow 1$ \textbf{to} $M$} \label{line:inner-loop}
            \STATE \textcolor{red}{\text{\# account for the contribution of $a_{\ell - 1, i}$ to $a_{\ell, i}$ - red cell}}
            \STATE \textcolor{red}{$a_{\ell, i} = \block^\ell(a_{\ell, i} + a_{\ell-1, i} \odot \rho_{\ell, 0})$} \label{line:red-tile}
            \STATE \textcolor{gray}{\text{\# account for the contribution of $a_{\ell - 1, [i - U + 1, i]}$ to $a_{\ell, [i + 1, i + U]}$ - gray tile}}
            \STATE \textcolor{gray}{$a_{\ell, [i + 1, i + U]} \pluseq \tau(a_{\ell-1}, [i - U + 1, i], \rho_\ell, [i + 1, i + U])$} \label{line:gray-tile}
        \ENDFOR
        \STATE \text{\# generate next token based on the output of last layer at position $i$}
        \STATE $a^0_{i + 1} = \sampler(a^M_{i})$
    \ENDFOR
\end{algorithmic}
\end{algorithm}
